A characterization of linear independence of THB-splines in $\mathbb{R}^n$ and application to B\'ezier projection

In this paper we propose a local projector for truncated hierarchical B-splines (THB-splines). The local THB-spline projector is an adaptation of the B\'ezier projector proposed by Thomas et al. (Comput Methods Appl Mech Eng 284, 2015) for B-splines and analysis-suitable T-splines (AS T-splines). For THB-splines, there are elements on which the restrictions of THB-splines are linearly dependent, contrary to B-splines and AS T-splines. Therefore, we cluster certain local mesh elements together such that the THB-splines with support over these clusters are linearly independent, and the B\'ezier projector is adapted to use these clusters. We introduce general extensions for which optimal convergence is shown theoretically and numerically. In addition, a simple adaptive refinement scheme is introduced and compared to Giust et al. (Comput. Aided Geom. Des. 80, 2020), where we find that our simple approach shows promise.

==> Images/Tikz/MainProjectionStepFigureBsplines/MatlabData.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{mycolor3}{rgb}{0.92900,0.69400,0.12500}%
%
\begin{tikzpicture}

\begin{axis}[%
width=10.333in,
height=2.143in,
at={(1.733in,3.667in)},
scale only axis,
xmin=0,
xmax=1,
ymin=-2,
ymax=1.06949116476744,
axis background/.style={fill=white}
]
\addplot [color=mycolor1, forget plot]
  table[row sep=crcr]{%
0.333285621128907	-0.920701310628476\\
0.333081991773266	-0.921634901945239\\
0.332715855788854	-0.923298869938259\\
0.332187489506241	-0.925666930180824\\
0.331497399207165	-0.928700918139481\\
0.330646256784343	-0.932351405125634\\
0.329634893081153	-0.936558142378938\\
0.328464295960618	-0.941250573767589\\
0.327135609042636	-0.94634843157771\\
0.325650130487582	-0.951762413291937\\
0.324009311689376	-0.957394934340639\\
0.322214755840513	-0.963140950718019\\
0.320268216357556	-0.968888844656048\\
0.318171595163755	-0.974521365990838\\
0.315926940828454	-0.979916621384736\\
0.31353644656417	-0.984949103171128\\
0.311002448082861	-0.989490749265818\\
0.308327421313265	-0.993412025339997\\
0.3055139799814	-0.996583020276487\\
0.302564873056529	-0.998874545834386\\
0.299482982065052	-1.00015923142796\\
0.296271318274916	-1.00031260498373\\
0.292933019753285	-0.999214150974675\\
0.289471348300337	-0.996748336940465\\
0.285889686262176	-0.99280560008699\\
0.282191533225967	-0.98728328591288\\
0.278380502600523	-0.980086531233734\\
0.274460318085688	-0.971129084461545\\
0.270434810033951	-0.960334056543479\\
0.266307911707863	-0.947634596565914\\
0.262083655436897	-0.932974486681066\\
0.257766168677516	-0.916308651709065\\
0.253359669980294	-0.897603579501788\\
0.248868464868032	-0.876837648919852\\
0.244296941628893	-0.854001363064085\\
0.239649567028672	-0.829097486210849\\
0.234930881946384	-0.802141083719594\\
0.230145496937438	-0.773159465003993\\
0.225298087728737	-0.742192030477736\\
0.220393390650088	-0.709290024195543\\
0.215436198006412	-0.674516194702085\\
0.210431353395251	-0.637944367369584\\
0.205383746974162	-0.599658932242171\\
0.200298310682623	-0.559754252105362\\
0.195180013423101	-0.518333996156239\\
0.190033856206019	-0.475510405258495\\
0.184864867263344	-0.431403495321207\\
0.179678097135573	-0.386140205836419\\
0.174478613736932	-0.33985350104407\\
0.169271497403591	-0.292681431559949\\
0.164061835929743	-0.244766164600098\\
0.158854719596401	-0.196252991161049\\
0.153655236197761	-0.147289318667631\\
0.14846846606999	-0.0980236576776926\\
0.143299477127314	-0.0486046112354939\\
0.138153319910233	0.0008201246071654\\
0.133035022650711	0.0501047407298775\\
0.127949586359171	0.0991062671900399\\
0.122901979938083	0.147685489914409\\
0.117897135326921	0.195707824331558\\
0.112939942683245	0.243044138863684\\
0.108035245604596	0.289571521679508\\
0.103187836395895	0.33517398464959\\
0.0984024513869497	0.37974309903627\\
0.0936837663046614	0.423178558087288\\
0.0890363917044403	0.465388662379271\\
0.0844648684653015	0.50629072446847\\
0.0799736633530395	0.545811390145124\\
0.0755671646558176	0.583886874347932\\
0.0712496778964365	0.620463110569547\\
0.0670254216254702	0.655495813365859\\
0.062898523299382	0.688950454364144\\
0.0588730152476451	0.72080215294095\\
0.0549528307328098	0.751035483502973\\
0.0511418001073663	0.77964420204644\\
0.0474436470711573	0.806630895385956\\
0.0438619850329965	0.832006557126253\\
0.0404003135800488	0.855790095093592\\
0.0370620150584174	0.878007775542146\\
0.0338503512682809	0.898692609999292\\
0.030768460276804	0.917883691107433\\
0.0278193533519332	0.935625484254611\\
0.0250059120200681	0.951967082157801\\
0.0223308852504726	0.966961429868325\\
0.0197968867691636	0.980664527905562\\
0.0174063925048788	0.993134621391139\\
0.0151617381695784	1.00443138314961\\
0.0130651169757777	1.01461509876263\\
0.0111185774928201	1.02374586151188\\
0.00932402164395733	1.03188278502163\\
0.00768320284575138	1.03908324121736\\
0.00619772429069741	1.04540213095326\\
0.00486903737271562	1.05089119433392\\
0.00369844025218028	1.05559836736997\\
0.00268707654899049	1.05956719118115\\
0.00183593412616804	1.06283627954223\\
0.00114584382709276	1.06543885036503\\
0.000617477544479143	1.06740232786249\\
0.00025134156006736	1.06874803398895\\
4.77122044264533e-05	1.06949116476744\\
};
\addplot [color=mycolor2, forget plot]
  table[row sep=crcr]{%
0.66661895446224	-0.9807344471887\\
0.666415325106599	-0.980800927159266\\
0.666049189122187	-0.980919104705375\\
0.665520822839574	-0.981086580613219\\
0.664830732540499	-0.981299889858317\\
0.663979590117676	-0.981554561305172\\
0.662968226414486	-0.981845169706828\\
0.661797629293951	-0.982165396920622\\
0.660468942375969	-0.982508103088109\\
0.658983463820915	-0.982865407297603\\
0.657342645022709	-0.983228776995262\\
0.655548089173847	-0.98358912529203\\
0.653601549690889	-0.983936915227178\\
0.651504928497088	-0.984262269977064\\
0.649260274161788	-0.984555087936693\\
0.646869779897503	-0.984805161550902\\
0.644335781416194	-0.98500229873189\\
0.641660754646598	-0.98513644567038\\
0.638847313314733	-0.985197809829333\\
0.635898206389863	-0.98517698190194\\
0.632816315398386	-0.985065055519662\\
0.629604651608249	-0.984853743511373\\
0.626266353086618	-0.984535489541065\\
0.62280468163367	-0.984103573988877\\
0.619223019595509	-0.983552212988072\\
0.6155248665593	-0.982876649588667\\
0.611713835933857	-0.982073236086114\\
0.607793651419022	-0.981139506630256\\
0.603768143367285	-0.980074239314967\\
0.599641245041196	-0.97887750704179\\
0.59541698877023	-0.977550716550568\\
0.591099502010849	-0.976096635115767\\
0.586693003313627	-0.974519404517867\\
0.582201798201365	-0.972824542013981\\
0.577630274962226	-0.97101892814961\\
0.572982900362005	-0.969110781373199\\
0.568264215279717	-0.967109619535843\\
0.563478830270772	-0.965026208478946\\
0.55863142106207	-0.962872498031915\\
0.553726723983421	-0.960661545858872\\
0.548769531339745	-0.958407429706919\\
0.543764686728584	-0.956125148717662\\
0.538717080307496	-0.953830514567447\\
0.533631644015956	-0.951540033299238\\
0.528513346756434	-0.949270778799268\\
0.523367189539352	-0.947040258953809\\
0.518198200596677	-0.944866275594817\\
0.513011430468906	-0.942766779407086\\
0.507811947070265	-0.940759721023457\\
0.502604830736924	-0.938862899577832\\
0.497395169263076	-0.937093810018055\\
0.492188052929735	-0.935469490501613\\
0.486988569531094	-0.93400637120654\\
0.481801799403323	-0.932720125887582\\
0.476632810460648	-0.931625527493753\\
0.471486653243566	-0.930736309137785\\
0.466368355984044	-0.930065031671002\\
0.461282919692504	-0.929622959069016\\
0.456235313271416	-0.929419942774719\\
0.451230468660255	-0.929464316075924\\
0.446273276016578	-0.929762799516113\\
0.44136857893793	-0.930320418248864\\
0.436521169729228	-0.931140432150296\\
0.431735784720283	-0.932224279400178\\
0.427017099637995	-0.933571534131984\\
0.422369725037774	-0.935179878636214\\
0.417798201798635	-0.937045090480548\\
0.413306996686373	-0.939161044786087\\
0.408900497989151	-0.941519731771946\\
0.40458301122977	-0.944111289552054\\
0.400358754958804	-0.946924052039133\\
0.396231856632715	-0.949944611682741\\
0.392206348580978	-0.953157896641935\\
0.388286164066143	-0.95654726186975\\
0.3844751334407	-0.960094593467294\\
0.380776980404491	-0.963780425550911\\
0.37719531836633	-0.967584068767513\\
0.373733646913382	-0.971483749491825\\
0.370395348391751	-0.975456758645802\\
0.367183684601614	-0.979479608995599\\
0.364101793610137	-0.983528199706133\\
0.361152686685267	-0.987577986867905\\
0.358339245353401	-0.991604158656152\\
0.355664218583806	-0.995581813738875\\
0.353130220102497	-0.999486141518422\\
0.350739725838212	-1.00329260277115\\
0.348495071502912	-1.00697710924177\\
0.346398450309111	-1.01051620075297\\
0.344451910826153	-1.01388721840737\\
0.342657354977291	-1.01706847248707\\
0.341016536179085	-1.02003940369659\\
0.339531057624031	-1.0227807364471\\
0.338202370706049	-1.02527462294478\\
0.337031773585514	-1.02750477692442\\
0.336020409882324	-1.02945659596827\\
0.335169267459501	-1.03111727149432\\
0.334479177160426	-1.03247588579669\\
0.333950810877812	-1.03352349660097\\
0.333584674893401	-1.03425321660116\\
0.33338104553776	-1.03466039350575\\
};
\addplot [color=mycolor3, forget plot]
  table[row sep=crcr]{%
0.999952287795574	-1.62345567562154\\
0.999748658439933	-1.61457214648415\\
0.999382522455521	-1.59864749936633\\
0.998854156172907	-1.57577630955275\\
0.998164065873832	-1.54609896688575\\
0.997312923451009	-1.50979788947304\\
0.99630155974782	-1.46709597097864\\
0.995130962627284	-1.41825495759584\\
0.993802275709303	-1.36357358950777\\
0.992316797154249	-1.30338549404487\\
0.990675978356043	-1.23805684093028\\
0.98888142250718	-1.16798377619468\\
0.986934883024222	-1.09358965417605\\
0.984838261830422	-1.01532208890733\\
0.982593607495121	-0.933649847678101\\
0.980203113230836	-0.849059610775148\\
0.977669114749527	-0.762052622398598\\
0.974994087979932	-0.673141258525259\\
0.972180646648067	-0.582845538047937\\
0.969231539723196	-0.491689603858571\\
0.966149648731719	-0.400198200661599\\
0.962937984941583	-0.308893176203327\\
0.959599686419951	-0.218290032283952\\
0.956138014967003	-0.128894551385212\\
0.952556352928843	-0.0411995240031945\\
0.948858199892634	0.0443183991700374\\
0.94504716926719	0.127201707212653\\
0.941126984752355	0.207014859407771\\
0.937101476700618	0.283346925963734\\
0.93297457837453	0.35581402049217\\
0.928750322103564	0.424061507515997\\
0.924432835344182	0.487765970208079\\
0.920026336646961	0.546636925601869\\
0.915535131534698	0.600418276650456\\
0.91096360829556	0.648889492721299\\
0.906316233695339	0.691866512381845\\
0.90159754861305	0.729202364636433\\
0.896812163604105	0.760787507097919\\
0.891964754395404	0.786549881898216\\
0.887060057316755	0.806454692441002\\
0.882102864673079	0.82050390635737\\
0.877098020061917	0.828735492222412\\
0.872050413640829	0.831222399708918\\
0.866964977349289	0.828071294875916\\
0.861846680089767	0.819421064197795\\
0.856700522872686	0.805441102718356\\
0.85153153393001	0.786329403348831\\
0.846344763802239	0.762310465806165\\
0.841145280403599	0.733633044995953\\
0.835938164070257	0.700567759772758\\
0.83072850259641	0.663404583950425\\
0.825521386263068	0.622450242179292\\
0.820321902864427	0.578025533850362\\
0.815135132736656	0.530462608525122\\
0.809966143793981	0.480102216521725\\
0.804819986576899	0.427290958213865\\
0.799701689317377	0.372378555319469\\
0.794616253025838	0.315715166976203\\
0.789568646604749	0.257648772724651\\
0.784563801993588	0.198522643655343\\
0.779606609349912	0.138672921931025\\
0.774701912271263	0.0784263276809245\\
0.769854503062562	0.0180980108910681\\
0.765069118053616	-0.0420104356030441\\
0.760350432971328	-0.101612787563682\\
0.755703058371107	-0.16043981254418\\
0.751131535131968	-0.218240693997359\\
0.746640330019706	-0.274784247412868\\
0.742233831322484	-0.329859921605918\\
0.737916344563103	-0.383278580334198\\
0.733692088292137	-0.434873061500907\\
0.729565189966049	-0.484498513291122\\
0.725539681914312	-0.532032508666981\\
0.721619497399477	-0.577374941695973\\
0.717808466774033	-0.620447711187357\\
0.714110313737824	-0.661194199046588\\
0.710528651699663	-0.699578552609323\\
0.707066980246715	-0.735584781968637\\
0.703728681725084	-0.769215684945996\\
0.700517017934948	-0.80049161386392\\
0.697435126943471	-0.829449099642802\\
0.6944860200186	-0.856139349954269\\
0.691672578686735	-0.880626639208225\\
0.688997551917139	-0.902986609021365\\
0.68646355343583	-0.923304498504256\\
0.684073059171545	-0.941673324206214\\
0.681828404836245	-0.958192029868379\\
0.679731783642444	-0.97296362625332\\
0.677785244159487	-0.986093341243747\\
0.675990688310624	-0.997686800135013\\
0.674349869512418	-1.00784825558935\\
0.672864390957364	-1.01667888607955\\
0.671535704039382	-1.02427518083462\\
0.670365106918847	-1.03072742832266\\
0.669353743215657	-1.0361183241935\\
0.668502600792835	-1.04052171342669\\
0.667812510493759	-1.04400148046718\\
0.667284144211146	-1.04661060188896\\
0.666918008226734	-1.04839039090546\\
0.666714378871093	-1.04937019516289\\
};
\end{axis}

\begin{axis}[%
width=10.333in,
height=2.143in,
at={(1.733in,0.691in)},
scale only axis,
xmin=0,
xmax=1,
ymin=-2,
ymax=1.06966473898471,
axis background/.style={fill=white}
]
\addplot [color=black, forget plot]
  table[row sep=crcr]{%
0	1.06966473898471\\
0.0101010101010101	1.00328485375315\\
0.0202020202020202	0.936132390818555\\
0.0303030303030303	0.868292718115528\\
0.0404040404040404	0.799851203578657\\
0.0505050505050505	0.730893215142534\\
0.0606060606060606	0.661504120741748\\
0.0707070707070707	0.591769288310891\\
0.0808080808080808	0.521774085784554\\
0.0909090909090909	0.451603881097328\\
0.101010101010101	0.381344042183804\\
0.111111111111111	0.311079936978573\\
0.121212121212121	0.240896933416225\\
0.131313131313131	0.170880399431351\\
0.141414141414141	0.101115702958544\\
0.151515151515152	0.0316882119323927\\
0.161616161616162	-0.0373167057125112\\
0.171717171717172	-0.105813682041577\\
0.181818181818182	-0.173717349120213\\
0.191919191919192	-0.240942339013829\\
0.202020202020202	-0.307403283787833\\
0.212121212121212	-0.373014815507636\\
0.222222222222222	-0.437691566238645\\
0.232323232323232	-0.501348168046271\\
0.242424242424242	-0.563899252995922\\
0.252525252525253	-0.625259453153006\\
0.262626262626263	-0.685343400582934\\
0.272727272727273	-0.744065727351114\\
0.282828282828283	-0.801341065522956\\
0.292929292929293	-0.857084047163867\\
0.303030303030303	-0.911209304339259\\
0.313131313131313	-0.963631469114538\\
0.323232323232323	-1.01426517355512\\
0.333333333333333	-1.0630250497264\\
0.343434343434343	-1.10981498683956\\
0.353535353535354	-1.15449590268878\\
0.363636363636364	-1.19691797221402\\
0.373737373737374	-1.23693137035522\\
0.383838383838384	-1.27438627205235\\
0.393939393939394	-1.30913285224534\\
0.404040404040404	-1.34102128587415\\
0.414141414141414	-1.36990174787873\\
0.424242424242424	-1.39562441319903\\
0.434343434343434	-1.418039456775\\
0.444444444444444	-1.43699705354659\\
0.454545454545455	-1.45234737845376\\
0.464646464646465	-1.46394060643644\\
0.474747474747475	-1.4716269124346\\
0.484848484848485	-1.47525647138818\\
0.494949494949495	-1.47467945823713\\
0.505050505050505	-1.46974604792141\\
0.515151515151515	-1.46030641538096\\
0.525252525252525	-1.44621073555573\\
0.535353535353535	-1.42730918338569\\
0.545454545454545	-1.40345193381077\\
0.555555555555556	-1.37448916177092\\
0.565656565656566	-1.3402710422061\\
0.575757575757576	-1.30064775005626\\
0.585858585858586	-1.25546946026135\\
0.595959595959596	-1.20458634776132\\
0.606060606060606	-1.14784858749611\\
0.616161616161616	-1.08510635440569\\
0.626262626262626	-1.01620982342999\\
0.636363636363636	-0.941009169508976\\
0.646464646464647	-0.859354567582593\\
0.656565656565657	-0.771096192590792\\
0.666666666666667	-0.676084219473523\\
0.676767676767677	-0.574415205017052\\
0.686868686868687	-0.467171233392909\\
0.696969696969697	-0.355680770618936\\
0.707070707070707	-0.241272282712982\\
0.717171717171717	-0.125274235692887\\
0.727272727272727	-0.00901509557649559\\
0.737373737373737	0.106176671618345\\
0.747474747474748	0.218972599873793\\
0.757575757575758	0.328044223172002\\
0.767676767676768	0.432063075495128\\
0.777777777777778	0.529700690825328\\
0.787878787878788	0.619628603144756\\
0.797979797979798	0.70051834643557\\
0.808080808080808	0.771041454679922\\
0.818181818181818	0.82986946185997\\
0.828282828282828	0.875673901957868\\
0.838383838383838	0.907126308955773\\
0.848484848484849	0.92289821683584\\
0.858585858585859	0.921661159580226\\
0.868686868686869	0.902086671171084\\
0.878787878787879	0.862846285590571\\
0.888888888888889	0.802611536820844\\
0.898989898989899	0.720053958844054\\
0.909090909090909	0.613845085642362\\
0.919191919191919	0.482656451197919\\
0.929292929292929	0.325159589492885\\
0.939393939393939	0.140026034509412\\
0.94949494949495	-0.0740726797703422\\
0.95959595959596	-0.318465019364222\\
0.96969696969697	-0.594479450290076\\
0.97979797979798	-0.903444438565742\\
0.98989898989899	-1.24668845020907\\
1	-1.6255399512379\\
};
\end{axis}

\begin{axis}[%
width=13.333in,
height=6.281in,
at={(0in,0in)},
scale only axis,
xmin=0,
xmax=1,
ymin=0,
ymax=1,
axis line style={draw=none},
ticks=none,
axis x line*=bottom,
axis y line*=left
]
\end{axis}
\end{tikzpicture}%
